DI-Retinex: Digital-Imaging Retinex Theory for Low-Light Image Enhancement

Many existing methods for low-light image enhancement (LLIE) based on Retinex theory ignore important factors that affect the validity of this theory in digital imaging, such as noise, quantization error, non-linearity, and dynamic range overflow. In this paper, we propose a new expression called Digital-Imaging Retinex theory (DI-Retinex) through theoretical and experimental analysis of Retinex theory in digital imaging. Our new expression includes an offset term in the enhancement model, which allows for pixel-wise brightness contrast adjustment with a non-linear mapping function. In addition, to solve the lowlight enhancement problem in an unsupervised manner, we propose an image-adaptive masked reverse degradation loss in Gamma space. We also design a variance suppression loss for regulating the additional offset term. Extensive experiments show that our proposed method outperforms all existing unsupervised methods in terms of visual quality, model size, and speed. Our algorithm can also assist downstream face detectors in low-light, as it shows the most performance gain after the low-light enhancement compared to other methods.

==> img_tex/lolv1-1.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/146.png}
      \caption{Input}
      \label{fig:lolv1-1-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexNet/146_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv1-1-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RRDNet/146.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv1-1-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ZeroDCE++/146.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-1-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexDIP/146.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-1-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/SCI/146.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-1-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/NightEnhance/146.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-1-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/PairLIE/146.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv1-1-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ours_/146.png}
      \caption{Ours}
      \label{fig:lolv1-1-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/146.png}
      \caption{GT}
      \label{fig:lolv1-1-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{-10pt} 
% \setlength{\belowcaptionskip}{-10pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-1}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-10.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/547.png}
      \caption{Input}
      \label{fig:lolv1-10-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/547.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-10-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/547_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-10-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/547.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-10-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/547.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-10-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/547.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-10-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/547.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-10-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/547.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-10-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/547.png}
      \caption{Ours}
      \label{fig:lolv1-10-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/547.png}
      \caption{GT}
      \label{fig:lolv1-10-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-10}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-11.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/665.png}
      \caption{Input}
      \label{fig:lolv1-11-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/665.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-11-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/665_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-11-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/665.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-11-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/665.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-11-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/665.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-11-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/665.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-11-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/665.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-11-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/665.png}
      \caption{Ours}
      \label{fig:lolv1-11-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/665.png}
      \caption{GT}
      \label{fig:lolv1-11-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-11}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-12.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/669.png}
      \caption{Input}
      \label{fig:lolv1-12-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/669.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-12-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/669_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-12-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/669.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-12-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/669.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-12-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/669.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-12-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/669.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-12-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/669.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-12-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/669.png}
      \caption{Ours}
      \label{fig:lolv1-12-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/669.png}
      \caption{GT}
      \label{fig:lolv1-12-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-12}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-13.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/748.png}
      \caption{Input}
      \label{fig:lolv1-13-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/748.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-13-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/748_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-13-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/748.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-13-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/748.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-13-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/748.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-13-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/748.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-13-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/748.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-13-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/748.png}
      \caption{Ours}
      \label{fig:lolv1-13-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/748.png}
      \caption{GT}
      \label{fig:lolv1-13-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-13}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-14.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/778.png}
      \caption{Input}
      \label{fig:lolv1-14-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/778.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-14-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/778_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-14-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/778.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-14-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/778.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-14-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/778.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-14-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/778.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-14-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/778.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-14-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/778.png}
      \caption{Ours}
      \label{fig:lolv1-14-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/778.png}
      \caption{GT}
      \label{fig:lolv1-14-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-14}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-15.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/780.png}
      \caption{Input}
      \label{fig:lolv1-15-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/780.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-15-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/780_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-15-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/780.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-15-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/780.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-15-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/780.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-15-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/780.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-15-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/780.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-15-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/780.png}
      \caption{Ours}
      \label{fig:lolv1-15-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/780.png}
      \caption{GT}
      \label{fig:lolv1-15-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-15}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-4.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/23.png}
      \caption{Input}
      \label{fig:lolv1-4-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexNet/23_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv1-4-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RRDNet/23.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv1-4-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ZeroDCE++/23.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-4-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexDIP/23.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-4-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/SCI/23.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-4-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/NightEnhance/23.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-4-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/PairLIE/23.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv1-4-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ours_/23.png}
      \caption{Ours}
      \label{fig:lolv1-4-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/23.png}
      \caption{GT}
      \label{fig:lolv1-4-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-4}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-5.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/55.png}
      \caption{Input}
      \label{fig:lolv1-5-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexNet/55_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv1-5-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RRDNet/55.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv1-5-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ZeroDCE++/55.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-5-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/RetinexDIP/55.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-5-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/SCI/55.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-5-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/NightEnhance/55.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-5-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/PairLIE/55.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv1-5-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/ours_/55.png}
      \caption{Ours}
      \label{fig:lolv1-5-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/55.png}
      \caption{GT}
      \label{fig:lolv1-5-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-5}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-7.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/111.png}
      \caption{Input}
      \label{fig:lolv1-7-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/111.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-7-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/111_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-7-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/111.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-7-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/111.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-7-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/111.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-7-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/111.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-7-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/111.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-7-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/111.png}
      \caption{Ours}
      \label{fig:lolv1-7-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/111.png}
      \caption{GT}
      \label{fig:lolv1-7-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-7}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-8.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/179.png}
      \caption{Input}
      \label{fig:lolv1-8-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/179.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-8-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/179_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-8-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/179.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-8-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/179.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-8-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/179.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-8-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/179.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-8-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/179.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-8-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/179.png}
      \caption{Ours}
      \label{fig:lolv1-8-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/179.png}
      \caption{GT}
      \label{fig:lolv1-8-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-8}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv1-9.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/input/493.png}
      \caption{Input}
      \label{fig:lolv1-9-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE/493.png}
      \caption{ZeroDCE~\citep{guo2020zero}}
      \label{fig:lolv1-9-b}
  \end{subfigure}
  
%   \centering
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexNet/493_S.png}
%       \caption{RetinexNet~\citep{Chen2018Retinex}}
%       \label{fig:lolv1-9-c}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.496\linewidth}
%     \includegraphics[width=0.95\linewidth]{figs/lolv1/RRDNet/493.png}
%       \caption{RRDNet~\citep{zhu2020zero}}
%       \label{fig:lolv1-9-d}
%   \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ZeroDCE++/493.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv1-9-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/RetinexDIP/493.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv1-9-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/SCI/493.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv1-9-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/NightEnhance/493.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv1-9-h}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/ours_/493.png}
      \caption{Ours}
      \label{fig:lolv1-9-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.496\linewidth}
    \includegraphics[width=0.95\linewidth]{figs/lolv1/GT/493.png}
      \caption{GT}
      \label{fig:lolv1-9-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v1~\citep{Chen2018Retinex}.}
  \label{fig:lolv1-9}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv2-1.tex <==
\begin{figure*}[h]
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/input/low00765.png}
      \caption{Input}
      \label{fig:lolv2-1-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexNet/low00765_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv2-1-c}
  \end{subfigure}
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RRDNet/low00765.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv2-1-b}
  \end{subfigure}
  \hfill
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ZeroDCE++/low00765.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv2-1-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexDIP/low00765.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv2-1-f}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/SCI/low00765.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv2-1-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/NightEnhance/low00765.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv2-1-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/PairLIE/low00765.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv2-1-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ours_/low00765.png}
      \caption{Ours}
      \label{fig:lolv2-1-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/GT/normal00765.png}
      \caption{GT}
      \label{fig:lolv2-1-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{-9pt} 
% \setlength{\belowcaptionskip}{-7pt}
  \caption{A visual comparison of enhancement results on LOL-v2~\citep{yang2021sparse}. Please zoom in for better visualization. }
  \label{fig:lolv2-1}
  % \vspace{-2mm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv2-5.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/input/low00711.png}
      \caption{Input}
      \label{fig:lolv2-5-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexNet/low00711_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv2-5-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RRDNet/low00711.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv2-5-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ZeroDCE++/low00711.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv2-5-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexDIP/low00711.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv2-5-f}
  \end{subfigure}

  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/SCI/low00711.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv2-5-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/NightEnhance/low00711.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv2-5-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/PairLIE/low00711.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv2-5-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ours_/low00711.png}
      \caption{Ours}
      \label{fig:lolv2-5-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/GT/normal00711.png}
      \caption{GT}
      \label{fig:lolv2-5-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v2~\citep{yang2021sparse}. Please zoom in for better visualization. }
  \label{fig:lolv2-5}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv2-7.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/input/low00713.png}
      \caption{Input}
      \label{fig:lolv2-7-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexNet/low00713_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv2-7-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RRDNet/low00713.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv2-7-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ZeroDCE++/low00713.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv2-7-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexDIP/low00713.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv2-7-f}
  \end{subfigure}

  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/SCI/low00713.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv2-7-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/NightEnhance/low00713.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv2-7-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/PairLIE/low00713.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv2-7-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ours_/low00713.png}
      \caption{Ours}
      \label{fig:lolv2-7-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/GT/normal00713.png}
      \caption{GT}
      \label{fig:lolv2-7-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v2~\citep{yang2021sparse}. Please zoom in for better visualization. }
  \label{fig:lolv2-7}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv2-8.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/input/low00714.png}
      \caption{Input}
      \label{fig:lolv2-8-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexNet/low00714_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv2-8-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RRDNet/low00714.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv2-8-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ZeroDCE++/low00714.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv2-8-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexDIP/low00714.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv2-8-f}
  \end{subfigure}

  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/SCI/low00714.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv2-8-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/NightEnhance/low00714.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv2-8-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/PairLIE/low00714.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv2-8-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ours_/low00714.png}
      \caption{Ours}
      \label{fig:lolv2-8-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/GT/normal00714.png}
      \caption{GT}
      \label{fig:lolv2-8-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v2~\citep{yang2021sparse}. Please zoom in for better visualization. }
  \label{fig:lolv2-8}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/lolv2-9.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/input/low00715.png}
      \caption{Input}
      \label{fig:lolv2-9-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexNet/low00715_S.png}
      \caption{RetinexNet~\citep{Chen2018Retinex}}
      \label{fig:lolv2-9-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RRDNet/low00715.png}
      \caption{RRDNet~\citep{zhu2020zero}}
      \label{fig:lolv2-9-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ZeroDCE++/low00715.png}
      \caption{ZeroDCE++~\citep{li2021learning}}
      \label{fig:lolv2-9-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/RetinexDIP/low00715.png}
      \caption{RetinexDIP~\citep{zhao2021retinexdip}}
      \label{fig:lolv2-9-f}
  \end{subfigure}

  \centering
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/SCI/low00715.png}
      \caption{SCI~\citep{ma2022toward}}
      \label{fig:lolv2-9-g}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/NightEnhance/low00715.png}
      \caption{NightEnhance~\citep{jin2022unsupervised}}
      \label{fig:lolv2-9-h}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/PairLIE/low00715.png}
      \caption{PairLIE~\citep{fu2023pairlie}}
      \label{fig:lolv2-9-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/ours_/low00715.png}
      \caption{Ours}
      \label{fig:lolv2-9-i}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.196\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv2/GT/normal00715.png}
      \caption{GT}
      \label{fig:lolv2-9-j}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{A visual comparison of enhancement results on LOL-v2~\citep{yang2021sparse}. Please zoom in for better visualization. }
  \label{fig:lolv2-9}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/plot_joint_hist.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/r/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/r/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/r/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/r/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/g/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/g/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/g/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/g/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/b/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/b/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/b/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHist/lolv1/b/179.png}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{The statistical experiments for showing the existence of $\betam$. The first and second rows are low light and normally exposed images respectively. The rest three rows are joint histogram between the pair of low light and normally exposed images. The histograms are computed in R,G,B channels respectively. Please zoom in for better visualization. }
  \label{fig:plot_joint_hist}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> img_tex/plot_joint_hist_reverse.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/input/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/lolv1/GT/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/r/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/r/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/r/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/r/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/g/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/g/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/g/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/g/179.png}
  \end{subfigure}
  
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/b/780.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/b/665.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/b/146.png}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1\linewidth]{figs/jointHistReverse/lolv1/b/179.png}
  \end{subfigure}
% \setlength{\abovecaptionskip}{0pt} 
% \setlength{\belowcaptionskip}{-13pt}
  \caption{The statistical experiments for showing the existence of $\betam'$ with a small magnitude. The first and second rows are low light and normally exposed images respectively. The rest three rows are joint histogram between the pair of low light and normally exposed images. The histograms are computed in R,G,B channels respectively. Please zoom in for better visualization. }
  \label{fig:plot_joint_hist_reverse}
%   \vspace{-0.1cm}
\end{figure*}
% \vspace{-1cm}

==> sec_tex/resul_tex/gener.tex <==

\subsection{Generalizability of The Proposed Losses}

. We train other zero-shot learning methods

==> sec_tex/supple.tex <==

\section{Derivation of Eq.~\ref{eq::newllie_model}}\label{sec::derivationNewLLIE}

We have the expressions of DI-Retinex theory for both low light and normally exposed images as follows:
\begin{align*}
        \left\{
            \begin{aligned}
                \I_l &= \mathcal{G}\left(\L_l \prodm \R + \epsilonm_l\right) + \deltam_l + \Delta\I_l\\
                \I_h &= \mathcal{G}\left(\L_h \prodm \R + \epsilonm_h\right) + \deltam_h + \Delta\I_h.
            \end{aligned}
        \right. 
\end{align*}

Plug the expression of $\mathcal{G}$.

\begin{align*}
        \left\{
            \begin{aligned}
                \I_l &= \mu + \lambda\left(\L_l \prodm \R + \epsilonm_l\right)^{\gamma} + \deltam_l + \Delta\I_l\\
                \I_h &= \mu + \lambda\left(\L_h \prodm \R + \epsilonm_h\right)^{\gamma} + \deltam_h + \Delta\I_h.
            \end{aligned}
        \right. 
\end{align*}

By transforming the first expression, we have
\begin{equation*}
    \R = \left\{ \left[\frac{1}{\lambda}\left(\I_l - \deltam_l - \Delta\I_l - \mu\right) \right]^{\frac{1}{\gamma}} - \epsilonm_l\right\} \oslash \L_l.
\end{equation*}

Plug it into the expression of extended Retinex theory for normally exposed image. Suppose $\r=\L_h \oslash \L_l \ge \onem$. Then we have
\begin{equation*}
\begin{split}
    \I_h = &\lambda\left(\r \prodm  \left[\frac{1}{\lambda}\left(\I_l - \deltam_l - \Delta\I_l - \mu\right) \right]^{\frac{1}{\gamma}} - \r \prodm \epsilonm_l + \epsilonm_h\right)^{\gamma} \\
    & + \mu + \deltam_h + \Delta\I_h.
\end{split}
\end{equation*}

\noindent  According to the approximation that 
%
\begin{equation}\label{eq::approximation}
    (1+x)^n=1+nx ,
\end{equation}
%
\noindent when $x\rightarrow 0$ by Taylor expansion, we can get 
%
\begin{equation*}
\begin{split}
    \I_h \approx &\lambda\r^\gamma \prodm  \left[\frac{1}{\lambda}\left(\I_l - \deltam_l - \Delta\I_l - \mu\right) \right]^{}  \\
    & + \lambda \gamma \r^{\gamma-1} (\epsilonm_h - \r \prodm \epsilonm_l) \left[\frac{1}{\lambda}\left(\I_l - \deltam_l - \Delta\I_l - \mu\right) \right]^{\frac{\gamma-1}{\gamma}} \\
    & + \mu + \deltam_h + \Delta\I_h.
\end{split}
\end{equation*}

\noindent Let the second term be
%
$$T = \lambda \gamma \r^{\gamma-1} (\epsilonm_h - \r \prodm \epsilonm_l) \left[\frac{1}{\lambda}\left(\I_l - \deltam_l - \Delta\I_l - \mu\right) \right]^{\frac{\gamma-1}{\gamma}},$$ 
%
and use approximation in Eq.~\ref{eq::approximation}, thus we have 
%
\begin{equation*}
\begin{split}
    T &= \lambda^{\frac{1}{\gamma}} \gamma \r^{\gamma-1} (\epsilonm_h - \r \prodm \epsilonm_l) \left(\I_l - \deltam_l - \Delta\I_l - \mu\right)^{\frac{\gamma-1}{\gamma}} \\
    &\approx \lambda^{\frac{1}{\gamma}} \gamma \r^{\gamma-1} (\epsilonm_h - \r \prodm \epsilonm_l) \left[\I_l^{\frac{\gamma-1}{\gamma}} + {\frac{1-\gamma}{\gamma}}(\deltam_l + \Delta\I_l + \mu) \I_l^{\frac{-1}{\gamma}}\right].
\end{split}
\end{equation*}

\noindent Note that $\gamma \approx 0.5$, $\r \ge \onem$ and thus $\r^{\gamma-1} \le \onem$. The noise term $(\epsilonm_h - \r \prodm \epsilonm_l)$ is small. When $\I_l\in[1,255]$, we have $\I_l^{\frac{\gamma-1}{\gamma}} \le \onem$ and $\I_l^{\frac{-1}{\gamma}} \le \onem$, which ensures $T\rightarrow 0$ compared to the maximum intensity of $255$ for $\I_h$. When $\I_{l,i,j}=0$ at $(i,j)$-th pixel, $\L_{l,i,j}$ also equals zero and thus $\r_{i,j}=+\infty \Rightarrow \r_{i,j}^{\gamma-1}\rightarrow 0$. Besides, the probability of $\I_{l,i,j}$ exactly equaling to zero is extremely small among pixels in reality. 
The second term $T$ is thus much smaller than the other terms and can be safely omitted, which yields
%
\begin{equation*}
\begin{split}
    \I_h &\approx \r^\gamma \prodm \left(\I_l - \deltam_l - \Delta\I_l - \mu\right) + \mu + \deltam_h + \Delta\I_h\\
    &= \r^\gamma \prodm \I_l + \left[\mu + \deltam_h + \Delta\I_h - \r^\gamma \prodm \left( \deltam_l + \Delta\I_l + \mu\right)\right].
\end{split}
\end{equation*}

\noindent Therefore, we can obtain
%
\begin{align*}
    &\I_h \approx \alpham \I_l + \betam. \\
    \text{where} &\left\{
    \begin{aligned}
        \alpham &= \r^{\gamma} = \left(\L_h \oslash \L_l \right)^\gamma \\
        \betam &= \mu + \deltam_h + \Delta\I_h - \r^\gamma \prodm \left( \deltam_l + \Delta\I_l + \mu\right).
    \end{aligned}
    \right.
\end{align*}

\section{Derivation of Eq.~\ref{eq::reverseDegradation}}\label{sec::derivationReverseDegradation}
We want to show 
%
\begin{align*}
    &\I_l \approx \alpham' \I_h + \betam', \\
    \text{where} &\left\{
    \begin{aligned}
        \alpham' &= \r^{-\gamma} = \left(\L_l \oslash \L_h \right)^\gamma \\
        \betam' &= \mu + \deltam_l + \Delta\I_l - \r^{-\gamma} \prodm \left( \deltam_h + \Delta\I_h + \mu\right).
    \end{aligned}
    \right.
\end{align*}
%
Similar to the derivation of Eq.~\ref{eq::newllie_model},  we start from
%
\begin{align*}
        \left\{
            \begin{aligned}
                \I_l &= \mathcal{G}\left(\L_l \prodm \R + \epsilonm_l\right) + \deltam_l + \Delta\I_l\\
                \I_h &= \mathcal{G}\left(\L_h \prodm \R + \epsilonm_h\right) + \deltam_h + \Delta\I_h.
            \end{aligned}
        \right. 
\end{align*}
%
and we can get
%
\begin{equation*}
\begin{split}
    \I_l = &\lambda\left(\r^{-1} \prodm  \left[\frac{1}{\lambda}\left(\I_h - \deltam_h - \Delta\I_h - \mu\right) \right]^{\frac{1}{\gamma}} - \r^{-1} \prodm \epsilonm_h + \epsilonm_l\right)^{\gamma} \\
    & + \mu + \deltam_l + \Delta\I_l.
\end{split}
\end{equation*}
%
Then by using approximation in Eq.~\ref{eq::approximation} we have
%
\begin{equation*}
\begin{split}
    \I_l \approx &\lambda\r^{-\gamma} \prodm  \left[\frac{1}{\lambda}\left(\I_h - \deltam_h - \Delta\I_h - \mu\right) \right]^{}  \\
    & + \lambda \gamma \r^{1-\gamma} (\epsilonm_l - \r^{-1} \prodm \epsilonm_h) \left[\frac{1}{\lambda}\left(\I_h - \deltam_h - \Delta\I_h - \mu\right) \right]^{\frac{\gamma-1}{\gamma}} \\
    & + \mu + \deltam_l + \Delta\I_l.
\end{split}
\end{equation*}
%
Let the second term be
%
\begin{equation*}
\begin{split}
    T' &= \lambda^{\frac{1}{\gamma}} \gamma \r^{1-\gamma} (\epsilonm_l - \r^{-1} \prodm \epsilonm_h) \left(\I_h - \deltam_h - \Delta\I_h - \mu\right)^{\frac{\gamma-1}{\gamma}} \\
    &\approx \lambda^{\frac{1}{\gamma}} \gamma \r^{1-\gamma} (\epsilonm_l - \r^{-1} \prodm \epsilonm_h) \left[\I_h^{\frac{\gamma-1}{\gamma}} + {\frac{1-\gamma}{\gamma}}(\deltam_h + \Delta\I_h + \mu) \I_h^{\frac{-1}{\gamma}}\right].
\end{split}
\end{equation*}
%
Note that $\r \ge \onem$, and thus $\r^{-1} \ge \onem$. The noise term $(\epsilonm_l - \r^{-1} \prodm \epsilonm_h)$ is small. When $\I_h\in[1,255]$, we have $\I_h^{\frac{\gamma-1}{\gamma}} \le \onem$ and $\I_h^{\frac{-1}{\gamma}} \le \onem$, which ensures $T\rightarrow 0$ compared to the maximum intensity. When $\I_{h,i,j}=0$ at $(i,j)$-th pixel, $\L_{h,i,j}$ also equals zero and thus $\r_{i,j}^{1-\gamma}\rightarrow 0$. Besides, the probability of $\I_{h,i,j}$ exactly equaling to zero is extremely small among pixels in reality. 
The second term $T'$ is thus much smaller than the other terms and can be safely omitted, which yields
%
\begin{equation*}
\begin{split}
    \I_l &\approx \r^{-\gamma} \prodm \left(\I_h - \deltam_h - \Delta\I_h - \mu\right) + \mu + \deltam_l + \Delta\I_l\\
    &= \r^{-\gamma} \prodm \I_h + \left[ \mu + \deltam_l + \Delta\I_l - \r^{-\gamma} \prodm \left( \deltam_h + \Delta\I_h + \mu\right) \right].
\end{split}
\end{equation*}
%
Therefore, we can obtain
%
\begin{align*}
    &\I_l \approx \alpham' \I_h + \betam. \\
    \text{where} &\left\{
    \begin{aligned}
        \alpham' &= \r^{-\gamma} = \left(\L_l \oslash \L_h \right)^\gamma \\
        \betam' &= \mu + \deltam_l + \Delta\I_l - \r^{-\gamma} \prodm \left( \deltam_h + \Delta\I_h + \mu\right).
    \end{aligned}
    \right.
\end{align*}


% Plug in the expression of $\mathcal{G}(x)=x^\gamma$ and thus $f^{-1}(x)=x^{\frac{1}{\gamma}}$, we can obtain
% \begin{equation*}
%     \R = \left(\left(\I_l - \deltam_l - \epsilonm_{r,l}\right)^{\frac{1}{\gamma}} - \epsilonm_{pd,l}\right) \oslash \L_l
% \end{equation*}

% Through the approximation that $(1+x)^n=1+nx$ when $x\rightarrow 0$ by Taylor expansion, we can get 
% \begin{equation*}
% \begin{split}
%     \R &= \left(\I_l^{\frac{1}{\gamma}}\left(1 - {\frac{1}{\gamma}} \frac{\deltam_l + \epsilonm_{r,l}}{\I_l}\right) - \epsilonm_{pd,l}\right) \oslash \L_l \\
%     &= \left(\I_l^{\frac{1}{\gamma}} - {\frac{1}{\gamma}} \left(\deltam_l + \epsilonm_{r,l}\right) \I_l^{\frac{1-\gamma}{\gamma}} - \epsilonm_{pd,l}\right) \oslash \L_l \\
% \end{split}
% \end{equation*}

% \noindent where $\frac{\deltam_l + \Delta\I_l + \mu}{\I_l}$ is small.


% the common term of reflectance $\R$ and supposing $\r = \L_h \oslash \L_l$, we obtain

% \begin{equation*}
%     \I_h = f\left(\r \prodm f^{-1}(\I_l - \deltam_l - \epsilonm_{r,l}) - \r \prodm \epsilonm_{pd,l} + \epsilonm_{pd,h}\right) + \deltam_h + \epsilonm_{r,h}.
% \end{equation*}

% Plug in the expression of $f(x)=x^\gamma$ and $f^{-1}(x)=x^{\frac{1}{\gamma}}$, we have 
% \begin{equation*}
%     \I_h = \left(\r \prodm (\I_l - \deltam_l - \epsilonm_{r,l})^{\frac{1}{\gamma}} - \r \prodm \epsilonm_{pd,l} + \epsilonm_{pd,h}\right)^\gamma + \deltam_h + \epsilonm_{r,h}.
% \end{equation*}

% By the approximation that $(1+x)^n=1+nx$ when $x\rightarrow 0$. We get 
% \begin{equation*}
% \begin{split}
%     \I_h &\approx \left(\r \prodm \left(\I_l^{\frac{1}{\gamma}} (1 - {\frac{1}{\gamma}}\frac{\deltam_l + \epsilonm_{r,l}}{\I_l}) \right) - \r \prodm \epsilonm_{pd,l} + \epsilonm_{pd,h}\right)^\gamma + \deltam_h + \epsilonm_{r,h}\\
%     &= \left(\r \prodm \left(\I_l^{\frac{1}{\gamma}} (1 - {\frac{1}{\gamma}}\frac{\deltam_l + \epsilonm_{r,l}}{\I_l}) \right) - \r \prodm \epsilonm_{pd,l} + \epsilonm_{pd,h}\right)^\gamma + \deltam_h + \epsilonm_{r,h}.
% \end{split}
% \end{equation*}

% \begin{align}
%     &\I_h \approx \alpham \I_l + \betam. \\
%     \text{where} &\left\{
%     \begin{aligned}
%         \r &= \L_h \oslash \L_l \\
%         \alpham &= \r^\gamma + \gamma \r^{\gamma-1} \left(\epsilonm_{h,pd}-\r \epsilonm_{l,pd}\right)  \\
%         \betam &= \deltam_h + \epsilonm_{h,r}- \r^\gamma (\deltam_l + \epsilonm_{l,r}),
%     \end{aligned}
%     \right.
% \end{align}


\section{Discussion of Linear Model and the Offset $\betam$}\label{sec::discussionBeta}
\subsection{Theoretical Analysis}
The expression of $\betam$ is given by
%
$$\betam = \mu + \deltam_h + \Delta\I_h - \alpham \prodm \left(\mu + \deltam_l + \Delta\I_l\right),$$
%
\noindent where $\alpham=\left(\L_h \oslash \L_l \right)^\gamma \ge \onem$. We analyse the magnitude of $\betam$ by computing its mean and variance. Given $\mathbb{E}[\alpham] =\overline{\alpham} > 1$ and $\mathbb{E}[\deltam_l]=\mathbb{E}[\deltam_h]=0$ and suppose $\alpham$ is independent of $\Delta\I_h$ and $\Delta\I_l$, we have
%
$$\mathbb{E}[\betam] = \mu(1-\overline{\alpham} ) + \mathbb{E}[\Delta\I_h] - \overline{\alpham}\mathbb{E}[\Delta\I_l] .$$
%
A properly exposed has equal probability of overexposure and underexposure. Thus $\mathbb{E}[\Delta\I_h] = 0$. Also a negative overflow exceeding $0$ caused by a negative image irradiance is seldom and thus $\mathbb{E}[\Delta\I_l]\rightarrow 0$. $\mu$ is a negative number such that the Gamma transformation can map $[0, +\infty)$ to $[0,255]$. $(1-\overline{\alpham}) < -1$ (found in the following statistical experiments) makes the magnitude of $\mathbb{E}[\betam]$ significant. Even if $\mu(1-\overline{\alpham} ) = \overline{\alpham}\mathbb{E}[\Delta\I_l]$ in some rare case, $\Delta\I_l$ has non-zero values only in some regions of an image and $\mu(1-\overline{\alpham} )$ has large values in the regions where $\Delta\I_l$ has zero values. Therefore, $\betam$ is not negligible in terms of considerable mean.

We then compute $\betam$'s variance. The variance of $\mu$ is zero as it is a constant. Since the quantization error follows a uniform distribution from $\-q/2$ to $q/2$, its variance is $q^2/12$. Note that with the assumption of flux consistency along time dimension across spatial pixels during receiving radiance in a short period, $\alpham$ can be further treated as a constant matrix. So it can be considered as a scalar $\alpha$ when computing $\betam$'s variance,
%
\begin{equation*}
\begin{split}
    Var(\betam) &= (q^2/12) + Var(\Delta\I_h) +\alpha^2 \left((q^2/12) + Var(\Delta\I_l) \right) \\
    &= (1+\alpha^2) (q^2/12) + Var(\Delta\I_h) + \alpha^2Var(\Delta\I_l).
\end{split}
\end{equation*}
%
As shown, the factor of $\alpha^2$ enlarges the variance of $\betam$. The amplified variance also makes $\betam$ non-negligible.

\subsection{Experimental Analysis}

We also conduct statistical experiments on the low light and normally exposed image pairs from LOL-v1~\citep{Chen2018Retinex}. For each pair, we plot the joint histogram of paired pixels in each channel as shown in Fig.~\ref{fig:plot_joint_hist}. The dots in orange are those of $\I \in (0, k)$ and the dots in light blue are those of $\I = k$ or $\I = 0$  representing the pixels may have dynamic range overflow. A linear regression of $\I_h=\alpham \I_l + \betam$ is done for the dots $\I_h < k$. The regressed line is plotted in red and its coefficients are attached beside the line. The regression is fitted well by the linear model with a $R^2$ close to 1. For most cases $\betam$ is of a large magnitude. Therefore, a non-negligible offset $\betam$ is shown in the experiments.

\input{img_tex/plot_joint_hist}

%Since $\deltam_l, \deltam_h \in [-\frac{q}{2}, \frac{q}{2}]$, $$\betam \in [\frac{q}{2}(-1-\alpham), \frac{q}{2}(1+\alpham)]$$

\newpage

\section{Discussion on Reverse Degradation}\label{sec::discussionBetaPrime}

\subsection{Theoretical Analysis}

The expression of $\betam'$ is given by
%
$$\betam' = \mu + \deltam_l + \Delta\I_l - \alpham' \prodm \left(\mu + \deltam_h + \Delta\I_h\right),$$
%
\noindent where $\alpham'=\left(\L_l \oslash \L_h \right)^\gamma \le \onem$. We analyse the magnitude of $\betam'$ by computing its mean and variance. Given $\mathbb{E}[\alpham'] =\overline{\alpham'} \in [0,1]$ and $\mathbb{E}[\deltam_h]=\mathbb{E}[\deltam_l]=0$ and suppose $\alpham'$ is independent of $\Delta\I_h$ and $\Delta\I_l$, we have
%
$$\mathbb{E}[\betam'] = \mu(1-\overline{\alpham'} ) + \mathbb{E}[\Delta\I_l] - \overline{\alpham'}\mathbb{E}[\Delta\I_h].$$
%
A properly exposed has equal probability of overexposure and underexposure. Thus $\mathbb{E}[\Delta\I_h] = 0$. Also a negative overflow exceeding $0$ caused by a negative image irradiance is seldom and thus $\mathbb{E}[\Delta\I_l]\rightarrow 0$. $\mu$ is a negative number such that the Gamma transformation can map $[0, +\infty)$ to $[0,255]$. $1-\overline{\alpham'}\in [0,1]$. This makes $\mathbb{E}[\betam'] \approx \mu(1-\overline{\alpham'} )$ getting small. %Therefore, $\betam'$ is negligible. 
For even more safely removing $\betam'$, we compute reverse degradation loss in Gamma space by taking a power of $\frac{1}{\gamma}$, which suppresses the magnitude of $\betam'$.

We then compute the variance of $\betam'$. Similar to Section~\ref{sec::discussionBeta}, we can get
%
\begin{equation*}
\begin{split}
    Var(\betam) &= (q^2/12) + Var(\Delta\I_l) +\alpha'^2 \left((q^2/12) + Var(\Delta\I_h) \right) \\
    &= (1+\alpha'^2) (q^2/12) + Var(\Delta\I_l) + \alpha'^2Var(\Delta\I_h),
\end{split}
\end{equation*}
%
where $\alpha'$ is the scalar form of $\alpham$ under the assumption of flux consistency along time dimension across spatial pixels during receiving radiance in a short period. As shown, the factor of $\alpha'^2$ is small as $\alpha'<1$. The variance of $\betam'$ is close to $(q^2/12) + Var(\Delta\I_l)$, which is the variance of error and offset terms in low light image. The value of variance is restricted.

\subsection{Statistical Experiments}

We also conduct statistical experiments on the low light and normally exposed image pairs from LOL-v1~\citep{Chen2018Retinex}. For each pair, we plot the joint histogram of paired pixels in each channel as shown in Fig.~\ref{fig:plot_joint_hist_reverse}. The dots in orange are those of $\I \in (0, k)$ and the dots in light blue are those of $\I = k$ or $\I = 0$  representing the pixels may have dynamic range overflow. A linear regression of $\I_l=\alpham \I_h + \betam'$ is done for the dots $\I_h \in (0,k)$. The regressed line is plotted in red and its coefficients are attached beside the line. The regression is fitted well by the linear model with a large $R^2$. For most cases $\betam'$ is of a small magnitude. Therefore, a negligible offset $\betam'$ is shown in the experiments.

\input{img_tex/plot_joint_hist_reverse}


\section{Discussion on Mapping Function $g$ and Contrast Brightness Algorithm}\label{sec::MappingFunc_g}

We use four nonlinear function mapping $[-1,1]$ to $[0, +\infty)$. According to the finding of statistical experiments in Section~\ref{sec::discussionBeta}. The ratio between the exposures of low light and normally exposed images is mainly within $[1,10]$, we thus make sure that most output values of mapping function lie in the region. The formula of four used functions are given below and their curves are drawn in Fig.~\ref{fig:compare_g}.
%
\begin{equation*}
    \begin{split}
        g (c) &= \tan\left( \frac{45 + (45 - \tau) c}{180} \pi \right) \\
        g_1 (c) &= \frac{1+c}{1-c + e} \\ 
        g_2 (c) &= 3\tanh^{-1}\left(\frac{1}{2} + \frac{1}{2}c\right) = \frac{3}{2}\log(\frac{3+c}{1-c + e}) \\
        g_3 (c) &= 3 \log(g(c) + 1).
    \end{split}
\end{equation*}
%
A shifted reciprocal function like $g_1$ is a straightforward and common choice. But we can see that $g_1$ has an extremely steep rise when $c>0.8$ and thus generates the worst result in Table.~\ref{tab:ablation}. To alleviate the steep rise, we apply a logarithm function to shifted $g_1$ and form $g_2$. It coincidentally becomes a shifted inverse hyperbolic tangent function. But it still cannot lead to a good enough performance. Then we choose a tangent function $g$ and its performance is satisfactory. We further try its logarithm $g_3$ with a gentler slope. It has even better effect but the nesting of two nonlinear functions yields more computations. Considering the trade-off, we just use $g$. %Note that the mapping function is not what we proposed.

\input{img_tex/compare_g}

% Note that the formulation of Eq.~\ref{eq::contrastbrightness3} is not what we propose originally. 
The majority of existing works about image contrast enhancement are based on histogram equalization~\citep{padmavathy2018image,vijayalakshmi2020comprehensive,Park2018ContrastEF}. Though some variants of Eq.~\ref{eq::contrastbrightness3} is used empirically in industry for adjusting image's contrast, there is no academic paper discussing it to the best of our knowledge. One of our contributions lies in employing it to solve low light enhancement problem with the zero-reference regulation of two losses. Compared with other functions with single coefficient, the formula involving two coefficients is more difficult for a neural network to learn. Our derived reverse degradation loss and variance suppression loss can effectively guide the network to learn the coefficient pair of the adjustment function. We experiment various mapping functions $g$ aforementioned and modified the original formulation with the best choice of $g$. 




% \newpage
\section{More Visual Results}\label{sec::moreResults}

We provide multiple more samples from LOL-v1~\citep{Chen2018Retinex}, LOL-v2~\citep{yang2021sparse}, and DARK FACE~\citep{yuan2019ug} from Fig.~\ref{fig:lolv1-1} to Fig.~\ref{fig:darkface-4}.

% NightEnhance~\citep{jin2022unsupervised} tend to blur.
\input{img_tex/lolv1-1}
\input{img_tex/lolv1-3}
% \input{img_tex/lolv1-4}
% \input{img_tex/lolv1-5}
\input{img_tex/lolv1-6}
\input{img_tex/lolv1-7}
\input{img_tex/lolv1-8}
\input{img_tex/lolv1-9}
\input{img_tex/lolv1-10}
% \input{img_tex/lolv1-11}
\input{img_tex/lolv1-12}
\input{img_tex/lolv1-13}
\input{img_tex/lolv1-14}
% \input{img_tex/lolv1-15}

\input{img_tex/lolv2-2}
\input{img_tex/lolv2-3}
% \input{img_tex/lolv2-4}
\input{img_tex/lolv2-5}
% \input{img_tex/lolv2-6}
\input{img_tex/lolv2-7}
% \input{img_tex/lolv2-8}
\input{img_tex/lolv2-9}

\input{img_tex/darkface-2}
\input{img_tex/darkface-3}
\input{img_tex/darkface-4}



==> tab_tex/abla_comp_g.tex <==
% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{figure}
\begin{minipage}[b]{0.49\linewidth}
\centering
 \includegraphics[scale=0.27]{figs/compare_g.png}
 \caption{f}
 \end{minipage}
 \begin{minipage}[b]{0.49\linewidth}
 \tabcolsep=0.01cm
\scriptsize
  \centering
  \caption{The LLIE performance of our small model with various settings on LOL-v1~\citep{Chen2018Retinex}.}
    \begin{tabular}{ccccc}
    \toprule
          & w/o $\betam$ & w/o $\mathcal{L}_{VS}$ & w/o $\mathcal{L}_{RD}$ & w/o $\mathcal{M}$ \\
    \midrule
    PSNR  & 6.44 & 17.52 & 13.47 & 18.44 \\
    SSIM  & 0.349 & 0.610 & 0.565 & 0.616 \\
    \midrule
          & $g_1$    & $g_2$    & $g_3$    & Ours \\
    \midrule
    PSNR  & 13.38 & 17.58 & \textbf{18.51} & 18.45 \\
    SSIM  & 0.587 & 0.597 & 0.617 & \textbf{0.630} \\
    \bottomrule
    \end{tabular}%
  \label{tab:ablation}%
% \end{table}%
\end{minipage}
\end{figure}

==> tab_tex/tab_ablat.tex <==
% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{table}[htbp]
\small
  \centering
  \caption{The LLIE performance of our small model with various settings on LOL-v1~\citep{Chen2018Retinex}.}
  \vspace{-3mm}
    \begin{tabular}{ccccc}
    \toprule
          & w/o $\betam$ & w/o $\mathcal{L}_{VS}$ & w/o $\mathcal{L}_{RD}$ & w/o $\mathcal{M}$ \\
    \midrule
    PSNR  & 6.442 & 17.519 & 13.486 & 18.442 \\
    SSIM  & 0.349 & 0.610 & 0.565 & 0.616 \\
    \midrule
          & $g_1$    & $g_2$    & $g_3$    & Ours \\
    \midrule
    PSNR  & 13.384 & 17.584 & \textbf{18.507} & 18.445 \\
    SSIM  & 0.587 & 0.597 & 0.617 & \textbf{0.630} \\
    \bottomrule
    \end{tabular}%
  \label{tab:ablation}%
  \vspace{-3mm}
\end{table}%


==> tab_tex/tab_sota_compare.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\vspace{-4.1mm}
\begin{table}[htbp]
\renewcommand{\arraystretch}{0.4}
\setlength\tabcolsep{4.pt}
\captionsetup{font={footnotesize}}
\scriptsize
  \centering
  \caption{Performance of ours and the baselines on LOL-v1.}
\vspace{-4mm}
    \begin{tabular}{ccccccc}
    \toprule
          & SNR   & MIRNet & DCC-Net & URetinex & Ours & Ours$_{SL}$\\
    \midrule
    PSNR[dB] & 24.61 & 24.14 & 22.72 & 21.33 & 21.54 & 24.47\\
    Size[M] & 39.12 & 31.79 & 13.19 & 0.34  & 0.04 & 0.04 \\
    \bottomrule
    \end{tabular}%
  \label{tab:sota_compare}%
  \vspace{-4.1mm}
\end{table}%

